Did Aristotle Use a Laptop? A Question Answering Benchmark with Implicit Reasoning Strategies

A key limitation in current datasets for multi-hop reasoning is that the required steps for answering the question are mentioned in it explicitly. In this work, we introduce StrategyQA, a question answering (QA) benchmark where the required reasoning steps are implicit in the question, and should be inferred using a strategy. A fundamental challenge in this setup is how to elicit such creative questions from crowdsourcing workers, while covering a broad range of potential strategies. We propose a data collection procedure that combines term-based priming to inspire annotators, careful control over the annotator population, and adversarial filtering for eliminating reasoning shortcuts. Moreover, we annotate each question with (1) a decomposition into reasoning steps for answering it, and (2) Wikipedia paragraphs that contain the answers to each step. Overall, StrategyQA includes 2,780 examples, each consisting of a strategy question, its decomposition, and evidence paragraphs. Analysis shows that questions in StrategyQA are short, topic-diverse, and cover a wide range of strategies. Empirically, we show that humans perform well (87%) on this task, while our best baseline reaches an accuracy of $\sim$66%.

==> obsolete/01_introduction_before_alt.tex <==

\section{Introduction}
\label{sec:introduction}

Developing models that successfully reason over multiple parts of their input has attracted substantial attention recently, leading to the creation of many multi-step reasoning Question Answering (QA) benchmarks
~\cite{welbl2018constructing,talmor2018web,khashabi2018looking,yang2018hotpotqa,dua2019drop,suhr2019corpus,khot2020qasc}.

Commonly, the language of questions in such benchmarks \emph{explicitly} describes the process for deriving the answer. For instance (Figure~\ref{figure:intro}, Q2), the question \nl{Was Aristotle alive when the laptop was invented?} encapsulates the reasoning steps required for answering it; (1) \emph{When was the laptop invented?}, (2) \emph{When was Aristotle alive?}, and (3) \emph{Is the answer to step 1 smaller than the answer to step 2?}. Thus, deriving the reasoning process mostly requires understanding \emph{the question}.
However, real-life questions often involve \emph{implicit} reasoning. For example (Figure~\ref{figure:intro}, Q1), answering the question \nl{Did Aristotle use a laptop?} (Q2) requires the same steps, but the model must infer that the strategy for answering the question involves \emph{temporal} reasoning.


\begin{figure}
    \centering
    \includegraphics[scale=0.6,trim=0cm 0.5cm 0cm 0cm]{figures/intro.pdf}
    \caption{
        Questions in \strategyqa{} require \emph{implicit} decomposition into reasoning steps (e.g. Q1). This is in contrast to the multi-step questions that \emph{explicitly} specify the reasoning process  (e.g. Q2). We annotate every QA pair with its decomposition (D) and supporting evidence from Wikipedia (E).
    }
    \label{figure:intro}
\end{figure}

Implicit questions pose several challenges compared to their explicit counterparts. First, retrieving the context is difficult as there is little overlap between the question and context. Moreover, questions tend to be short, which lowers the possibility of the model exploiting shortcuts in the language of the question.

% In this work, we introduce \strategyqa{}, a benchmark for diverse and implicit multi-step reasoning QA. 
% Building a dataset of implicit multi-hop questions is challenging due to several reasons.
% First, as we are not looking for a particular reasoning pattern, it is not obvious what kind of questions should be collected. 
% \daniel{This does \emph{not} sound like a \strategyqa{}-specific challenge; \emph{any} dataset collection needs to ensure the diversity factor in the collection.}
% Considering the implicit questions in Table~\ref{table:example_strategy_questions}, they all need different reasoning procedures and they barely cover the space of possible implicit reasoning needed to answer questions. \jb{I think this is a bit unclear, see suggestion after next paragraph}

% Moreover, it is not clear how to collect implicit questions. Prior work has collected natural search-engine questions written by users \cite{kwiatkowski2019natural}, but is it possible to collect questions without users? Crowdsourcing has been a prevalent method for data collection, where crowdworkers are asked to write questions about a given context \mg{refs}. However, executing a crowdsourcing task for question writing at scale requires worker creativity and is prone to biases \mg{refs annotator bias and more}.

% To build \strategyqa{}, we characterize a type of questions termed ``strategy questions'', and design a priming method for inspiring worker creativity instead of providing workers with specific context. To further reduce biases, we integrate online solvers in the question writing task and create an annotator data-split.

In this work, we introduce \strategyqa{}, a benchmark for answering implicit multi-step reasoning questions, termed \emph{strategy questions} where a \emph{strategy} is the ability to infer from an implicit question its atomic sub-questions.
Collecting strategy questions requires overcoming several challenges. 
First, past work often collected multi-hop questions by presenting contexts to crowdsourcing workers and asking them to come up with questions. However, priming workers with contexts leads to high lexical overlap between questions and contexts and consequently to reasoning shortcuts. Datasets, such as Natural Questions \cite{kwiatkowski2019natural} and MS MARCO \cite{nguyen2016ms}, overcome this by using real user questions. However, is it possible elicit creative questions with no context without access to users, using crowdsourcing only?


Second, an important desired property in \strategyqa{} is that questions entail \emph{diverse} strategies. While the example in Figure~\ref{figure:intro} reasons about time, there are many possible strategies for answering questions (see Table~\ref{table:example_strategy_questions}). We would like a benchmark that exposes as many strategies as possible. However, crowdsourcing often involves workers that use repetitive patterns, which may limit question diversity. 
%\daniel{Consider switching the ordering of these two ``challenges'' (i.e., first talk about the ``priming'' issue, and then bring up the diversity aspect.)}

We develop a pipeline for eliciting strategy questions that overcomes the above difficulties: (a) we prime workers with random terms that serve as minimal content to inspire the imagination of crowd workers and increase creativity in question writing, (b) we use a large set of annotators to further increase diversity of our questions, and (c) we employ adversarial filtering, that is, we train models during data collection to minimize annotation artifacts (e.g., correlations between the question text and the labels). 

Moreover, \strategyqa{} comes with (a) \emph{decomposition} annotations, the sequence of the steps required for computing the answer to the question, (b) \emph{evidence} annotations, which ground \emph{each} decomposition step to a Wikipedia paragraph containing its answer. 
This is the first QA dataset to provide evidence annotations for each individual step of the reasoning process.

Evaluating state-of-the-art models on \strategyqa{} shows that... human evaluation \mg{highlight results from our experiments}.

In summary, our contributions in this work are: 
\begin{enumerate}
    \item Defining \emph{strategy} questions -- a class of natural language question that necessitate \emph{implicit} multi-step reasoning.
    \item The \strategyqa{} dataset, a challenging QA benchmark, consisting of \mg{x} examples.
    \item A novel priming method and infrastructure for creative question writing.
\end{enumerate}
The dataset and code are publicly available at \url{https://anonymous}.


==> obsolete/01_introduction_old.tex <==

\section{Introduction}
\label{sec:introduction}


Open-domain Question Answering (QA) is the way users acquire knowledge from large textual corpora, while using free-form natural language. 
State-of-the-art QA models hold extensive knowledge about language and the world \cite{peters2018elmo, devlin2018bert, liu2019roberta, petroni2019language, hewitt2019structural, roberts2020much}.
\daniel{not sure why you have \cite{hewitt2019structural} here. }
They could answer factoid questions such as \nl{When did Aristotle live?} and \nl{When was the laptop invented?}.
However, executing complex reasoning processes over text is still an out of reach capability \mg{refs?}. For example, models will probably fail to conclude that Aristotle did not use a laptop from the answers to the previous questions (\nl{384-322 BC} and \nl{1981}, respectively).
\daniel{
here we can define what we mean by `\emph{multi-step reasoning QA}'. 
}
This limitation enforces the user to interact with the model iteratively through simple questions, while reasoning over the retrieved information by herself. \tushar{I didn't quite get the purpose of starting the introduction with open-domain QA. It seems the key point is the \emph{implicit} multi-step reasoning, so we could just start with your next para to get to that point sooner. ``To push QA models beyond simple factoid QA, multi-hop QA datasets, that require models to combine information from multiple fact, have been proposed recently. However these datasets are designed by explicitly showing the facts that should be combined leading to questions that explicitly describe...''}

% \begin{figure}
%     \centering
%     % you can see and update the figures here: https://drive.google.com/file/d/1D--eAApVqvP1i7GmsRW_KmbucZBbyvUk/view?usp=sharing 
%     % Saw this comment only after creating another file :)
%     \includegraphics[scale=0.65,trim=0cm 0cm 0cm 0cm]{figures/intro.pdf}
%     \caption{TBD}
%     \label{fig:intro}
% \end{figure}
Multi-step reasoning QA datasets are usually built by crowdworkers who write questions based on a given context  \cite{rajpurkar2016squad,trischler2017newsqa,yang2018hotpotqa,dua2019drop, dasigi2019quoref}, or by following specific question patterns \cite{yang2018hotpotqa, khot2020qasc}.\tushar{I am not sure what do you mean by specific question patterns. One key restriction of these approaches: They create questions from pair of paras/sentences with shared entities. If you look at the two facts needed for these questions, there is no overlap.}
\daniel{
not sure why we call \cite{rajpurkar2016squad,trischler2017newsqa} as `Multi-step' datasets. 
}
This often leads to questions that \emph{explicitly} describe the answer derivation process. For instance, the question \nl{Was Aristotle born after the laptop was invented?} encodes the reasoning steps for answering it; 1) When was Aristotle born?, 2) When was the laptop invented?, and 3) Is the answer to step 1 before the answer to step 2? In other words, replacing entities in the question would not change the answer derivation process, indicating there is no implicit knowledge required to answer the question.
In contrast, decomposing the question \nl{Did Aristotle use a laptop?} into reasoning steps, requires the implicit knowledge that Aristotle lived in Ancient Greece.

Exposing the reasoning process during training of QA models induces two major issues. First, it provides additional information that does not exist in many natural open-domain questions \cite{kwiatkowski2019natural}. In addition, it can introduce shortcuts in the answer derivation process, leading to overestimation of model performance \cite{jiang2019avoiding, jia2017adversarial}.



\daniel{Part of the following paragraph could become the beginning of the current 2nd paragraph:}
In this work, we focus on multi-step questions where the reasoning process is \emph{implicit}.
We introduce \strategyqa{}, the first dataset for diverse and implicit multi-step reasoning QA.
Building such a dataset is challenging due to several reasons: 
First, as we are not looking for a particular reasoning pattern\tushar{It would help if we could clarify this a bit here. Something along the lines of: e.g., ``Can Aristotle use a laptop'',  ``Can avocadoes grow in Antarctica?'', ``Can one spot helium?'' all need different reasoning procedures and they barely cover the space of possible implicit reasoning needed to answer questions. }, it is not obvious what kind of questions should be collected.
Moreover, executing a crowdsourcing task for question writing at scale requires worker creativity and is prone to biases.
Last, evaluating whether a model executes the expected reasoning process requires redefinition of the QA setting.
To build \strategyqa{}, we characterize a type of questions termed ``strategy questions'', define a new QA setting for multi-step reasoning, and design a priming method for inspiring worker creativity.

Evaluating state-of-the-art models on \strategyqa{} shows that... human evaluation \mg{highlight results from our experiments}.


To conclude, our contributions in this work are: 
\begin{enumerate}
    \item A \mg{definition? description?} of a type of questions, called strategy questions, that require implicit multi-step reasoning
    \item The \strategyqa{} dataset, a challenging QA benchmark, consisting of \mg{x} examples.
    \item An infrastructure for multi-step data collection pipeline over crowdsourcing
    \item A novel priming method for creative question writing.
\end{enumerate}

The dataset and code are publicly available at \url{https://anonymous}. 


==> obsolete/03_reasoning_description.tex <==

\section{Answering Strategy Questions}
\label{sec:reasoning_description}

% \jb{maybe call this section `Decomposing Strategy Questions'? seems like that's the focus of it.} 
% \mg{I feel like ``decomposing'' is not enough because we also collect evidence for answering them. How about ``Answering Strategy Questions''?}
\tushar{To me this looks like "Defining Strategy Questions". It also might be worth combining with the previous section of the desiderata. Sec 2.1 could be the desiderata -- what kind of questions we want. 2.2. could be these annotations -- what kind of auxillary supervision/annotations do we want.}
% \daniel{I am not sure why this section is not part of S4.2.} 
% \mg{Here we describe *what* we want to collect - decompositions and evidence. Section 4 is about *how* we collect this. }

Strategy questions involve complex reasoning that leads to a boolean answer (\S\ref{sec:strategy_questions}).
% \daniel{
%     I think, questions leading to `boolean answers' was a \emph{design choice}, not an attribute of `strategy questions' (so that we focus on the inputs, by choosing a simple schema for the output space). If so, the sentence should be rephrased. 
%     One can 
%     We can also add a sentence about creating `strategy' with a broader output (and input) format as a potential future work in the conclusion section. 
% }
% \mg{Yes you are right, it is a design choice. We mention this just a few lines before this one, at the end of section 2. We mention it here in the context that the answer is a weak signal. I've added the point regarding future work to the conclusion section.}
To guide and evaluate the question answering process, we annotate every question-answer pair with a description of the expected reasoning process. 

Prior work often used \emph{rationales} or \emph{supporting facts}, which are text snippets that are usually extracted from the context \cite{deyoung2020eraser,yang2018hotpotqa, kwiatkowski2019natural}, as evidence for an answer. 
% \daniel{
% Not sure how  \cite{yang2018hotpotqa} and \cite{kwiatkowski2019natural} fit here. 
% }
% \mg{they both annotated supporting facts.}
However, reasoning can rely on information and operations (such as number comparison) that are not explicitly expressed in the context.
Moreover, answering a question based on the relevant context does not imply that the model performs reasoning properly \cite{jiang2019avoiding}. \jb{are the two points in the last two sentences actually one?}
% \daniel{how is knowing this important for us? Does it guide any of our design decisions?} \mg{this paragraph is for motivating our decomposition + evidence annotations, by saying that what people have done before is not enough.}

Inspired by recent work \cite{wolfson2020break}, we associate every question-answer pair with a \emph{strategy question decomposition}.
A decomposition of a question $q$ is a sequence of $n$ steps $\langle s^{(1)}, s^{(2)}, ..., s^{(n)} \rangle$ required for computing the answer to $q$. Each step $s^{(i)}$ is a sequence of tokens $s^{(i)} = \langle s^{(1)}_1, s^{(1)}_2,..., s^{(1)}_{|s^{(i)}|} \rangle$ corresponding to a single-step question. 
The tokens include special \emph{reference tokens}, which are placeholders referring to the result of a previous step $s^{(j)}$. The last decomposition step (i.e. $s^{(n)}$) always returns the final answer to the question. Table~\ref{table:decomposition_examples} shows question decomposition examples. \tushar{I don't see the need for tokens. Can we simplify this text to only mention the steps with possible references to answers to other steps?}

Prior work on question decomposition \cite{wolfson2020break} targeted explicit multi-step questions (first row in Table~\ref{table:decomposition_examples}), for which the decomposition uses a small vocabulary derived from the question.
Conversely, decomposing strategy questions requires using implicit knowledge that is not stated in the question. 
Therefore, decompositions can include any token that is needed for describing the implicit reasoning (rows 2-4 in Table~\ref{table:decomposition_examples}).

In this work, we distinguish between two types of steps. A \textit{retrieval step}: a step that requires retrieval from the corpus\tushar{This misses the question-answering aspect. How about: retrieval QA step: a step that requires answering a question by retrieving facts from a corpus}, and an \textit{operation step}, a logical function over answers to previous steps. \daniel{the current phasing implies that a step can be either (a) or (b), and not both at the same time. }\tushar{I think that is the case, right?}
In Figure~\ref{figure:intro}, the first two steps are retrieve steps about \nl{Aristotle} and \nl{laptop}, and the last step is an operation step that compares the previous answers.


% \jb{will we more precisely define strategy question decomposition in section 4? if yes, we should say that. If not, we should think if to make it a bit more precise here. Bottom line the reader needs at some point to precisely understand what are these question decompositions}

\begin{table}[t]
    \centering
    \footnotesize
    % \resizebox{.5\textwidth}{!}
    {
    \begin{tabular}{p{2.1cm}|p{4.5cm}}
    % \begin{tabular}{l|l}
        Question & Decomposition \\ \toprule
         \multirow{3}{=}{Did the Battle of Peleliu or the Seven Days Battles last longer?} & (1) How long did \textbf{the Battle of Peleliu last}? \\
         & (2) How long did \textbf{the Seven Days Battle last}? \\
         & (3) Which is \textbf{longer} of \#1 , \#2? \\ \midrule
         \multirow{3}{=}{Can the President of Mexico vote in New Mexico primaries?} & (1) What is \emph{the citizenship requirement} for \textbf{voting in} \textbf{New Mexico}? \\
         & (2) What is \emph{the citizenship requirement} of any \textbf{President of Mexico}? \\
         & (3) Is \#2 the same as \#1?  \\ \midrule
         \multirow{3}{=}{Do guitarist's have fingers that can handle pain better than average?} & (1) What typically \emph{forms on} a \textbf{Guitarists' finger}? \\
         & (2) Does \#1 usually \emph{cause a lack of sensation?} \\ & \\ \midrule
         \multirow{4}{=}{Can a microwave melt a Toyota Prius battery?} & (1) What \emph{kind of} \textbf{battery} does a \textbf{Toyota Prius} use? \\
         & (2) What \emph{type of material} is \#1 made out of? \\
         & (3) What is the \emph{melting point} of \#2?  \\
         & (4) Can a \textbf{microwave's} \emph{temperature} reach at least \#3?   
    \end{tabular}
    }
    \caption{Explicit (first row) versus strategy (second row) question decompositions. Text from the input is marked in bold, italic text marks words which are implicit from the input.}
    \label{table:decomposition_examples}
\end{table}


To verify that steps are valid single-step questions that can be answered using the corpus (Wikipedia), we collect
\textit{supporting evidence} for each retrieval step and mark operation steps.
A supporting evidence is one or more paragraphs from the corpus (Wikipedia) that provides an answer to the retrieval step.

In summary, each example in our dataset contains a) a strategy question, b) a strategy question decomposition, and c) supporting evidence for every decomposition. 
In the next section (\S\ref{sec:data_collection}), we explain our methodology for collecting strategy questions and their annotations.


==> obsolete/053_human_retrieval_performance.tex <==

\subsection{Human performance in finding evidence}
\label{subsection:human_retrieval_performance}

\mg{I'm not sure how to position this and where to put it - it uses the Recall@10 score defined in \S\ref{subsection:experiment_results}, which depends on \S\ref{subsec:human_performance}.}
To quantify human performance in finding evidence, we ask experts (authors) to find evidence paragraphs in our corpus for 100 random questions. For half of the questions we additionally provide the question decomposition. 
We observe average Recall@10 scores of $0.586$ and $0.513$ with and without having the decomposition, respectively. These results show that humans perform significantly better than our IR baselines, showing there is a room for improvement. However, humans are still far from covering the gold paragraphs matched by workers. This could be a result of the existence of multiple valid evidence (\S\ref{subsec:data_quality}), or the challenge in this task for humans. Lastly, using the decomposition helps finding the relevant context. \mg{should write this better...} \jb{Let's discuss?}



==> obsolete/05_baselines.tex <==

\section{Baseline Models}
\label{sec:baselines}

% Questions in \strategyqa{} require complex reasoning over multiple pieces of open-domain and commonsense knowledge (\S\ref{subsec:data_diversity}). This holds multiple challenges of a) inferring the answering strategy, b) retrieving the relevant context, and c) computing the answer from the context.
% Therefore, we use the following models for our experiments:

% \paragraph{QA models}
% State-of-the-art models for QA are pre-trained language models (LMs), fine-tuned on down-stream QA tasks. Therefore, we use \textsc{RoBERTa} \cite{liu2019roberta}, a pre-trained LM with high performance on many NLU benchmarks, as our base model. To further improve its reasoning and commonsense skills, we fine-tune it on three datasets:
Answering strategy questions requires extensive world and commonsense knowledge that cannot be obtained by training on \strategyqa{} only. Therefore, both our models and online solvers (\S\ref{subsection:cqw}) are based on pre-trained language models, fine-tuned on auxiliary datasets that require reasoning. Specifically, we take \textsc{RoBERTa} \cite{liu2019roberta} and fine-tune it on:
%in several configurations (Table~\ref{table:baseline_models}):
\begin{itemize}[leftmargin=*,topsep=5pt,itemsep=0pt,parsep=0pt]
    \item \textsc{BoolQ} \cite{clark2019boolq}: A large-scale dataset for boolean question answering.
    \item \textsc{MNLI} \cite{williams2018broad}: A large-scale natural language inference (NLI) dataset. Each example contains a premise and hypothesis, and the model predicts if the hypothesis entails, contradicts, or neutral with respect to the premise.
    \item \textsc{Twenty Questions} (\textsc{20Q}): A collection of 50K short commonsense boolean questions.\footnote{\url{https://github.com/allenai/twentyquestions}}
    \item \textsc{DROP} \cite{dua2019drop}: A large-scale dataset for numerical reasoning over paragraphs.
\end{itemize}
% We train 5 baseline models with different fine-tuning settings, summarized in Table~\ref{table:baseline_models}.
% For the online solvers integrated in the collection pipeline \S\ref{subsection:cqw}, we combine these models as \textsc{Ckpt0}, and the models that do not use context as \textsc{Fntd}.

Models are trained in two configurations:
\begin{itemize}[leftmargin=*,topsep=0pt,itemsep=0pt,parsep=0pt]
    \item \textbf{No context} (\textsc{RoBERTa}): The model is fed with the question only, and output a binary prediction using the \texttt{CLS} token.

    \item \textbf{With context} (\textsc{RoBERTa$_{\text{IRq}}$}, \textsc{RoBERTa$_{\text{IRd}}$}): We use the \textsc{\textsc{BM25}} method \cite{robertson1995almbox} to retrieve context from our corpus in two ways: a) by using the question as a query and taking the top $k=5$ \mg{check} results, and b) by initiating a separate query for each decomposition step and taking the top result for each step. The model is fed with both the question and the retrieved context, and output a binary prediction.\footnote{Due to space limitation, details on model training are not provided. We will release our codebase and the exact training details upon acceptance.}
\end{itemize}

Overall, we trained 8 models (Table~\ref{table:baseline_models}), out of which 5 were integrated as online solvers in the data collection process (\S\ref{subsection:cqw}). 


\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabular}{lc}
      Model  & Solver group(s) \\ \hline
      \textsc{RoBERTa}  &  \\
      \textsc{RoBERTa$_{IR}$}  &  \\
      \textsc{RoBERTa+20Q}  &  \ckptzero{}, \fntd{} \\
      \textsc{RoBERTa+20Q+BoolQ}  & \ckptzero{}, \fntd{} \\
      \textsc{RoBERTa+BoolQ}  &  \ckptzero{}, \fntd{} \\
      \textsc{RoBERTa$_{IR}$+BoolQ}  & \ckptzero{} \\
      \textsc{RoBERTa$_{IR}$+MNLI+BoolQ}  & \ckptzero{} \\
      \textsc{RoBERTa$_{IR}$+DROP+20Q+BoolQ}  & 
    \end{tabular}
    \caption{QA baseline models and the online solver groups they were used in (\S\ref{subsection:cqw}).
    Each model was fine-tuned on the datasets mentioned in its name, prior to fine-tuning on \strategyqa{}, e.g. \textsc{RoBERTa+MNLI+BoolQ} was first fine-tuned on \textsc{MNLI} and then on \textsc{BoolQ}.
    \textsc{RoBERTa$_{NC}$} }
    \label{table:baseline_models}
\end{table}



% \paragraph{Context retrieval}
% For all models that use context, we employ the \textsc{\textsc{BM25}} \cite{robertson1995almbox} and initiate \texttt{multi\_match} queries against the fields of paragraph text, page title and section header, while boosting the title by 3 and the header by 2. \jb{I don't think these retrieval details are important for the paper}
% \mg{should think how to write this part, and say how we choose the final context from the results.}
% Given a question $q$ and its decomposition steps $s_1, ..., s_n$, we compare several retrieval methods:
% \begin{itemize}[leftmargin=*,topsep=0pt,itemsep=0pt,parsep=0pt]
%     \item \textsc{Que}: A single query $q$.
%     \item \textsc{QueDec}: A single query that is a concatenation of the question and decomposition $q s_1 ... s_n$. \jb{at this point it is not clear how you have a decomposition, maybe first talk about the decomposition?}
%     \item \textsc{DecSteps}: Multiple queries, a query for each decomposition step. \jb{unclear, what is exactly done?}
% \end{itemize}


\paragraph{Predicting decompositions}
To assess the utility of question decompositions (\S\ref{sec:experiments}), we train a model that given a question, generates its decomposition token-by-token. Specifically, we take \textsc{BART} \cite{lewis2020bart} and fine-tune it on the decompositions from \strategyqa{}.
\mg{pre-training on BREAK?}

